Towards Open Respiratory Acoustic Foundation Models: Pretraining and Benchmarking

Respiratory audio, such as coughing and breathing sounds, has predictive power for a wide range of healthcare applications, yet is currently under-explored. The main problem for those applications arises from the difficulty in collecting large labeled task-specific data for model development. Generalizable respiratory acoustic foundation models pretrained with unlabeled data would offer appealing advantages and possibly unlock this impasse. However, given the safety-critical nature of healthcare applications, it is pivotal to also ensure openness and replicability for any proposed foundation model solution. To this end, we introduce OPERA, an OPEn Respiratory Acoustic foundation model pretraining and benchmarking system, as the first approach answering this need. We curate large-scale respiratory audio datasets (~136K samples, over 400 hours), pretrain three pioneering foundation models, and build a benchmark consisting of 19 downstream respiratory health tasks for evaluation. Our pretrained models demonstrate superior performance (against existing acoustic models pretrained with general audio on 16 out of 19 tasks) and generalizability (to unseen datasets and new respiratory audio modalities). This highlights the great promise of respiratory acoustic foundation models and encourages more studies using OPERA as an open resource to accelerate research on respiratory audio for health. The system is accessible from https://github.com/evelyn0414/OPERA.

==> sections/01intro_old.tex <==


% \begin{figure}[h]
%     \centering
%     \includegraphics[height = 3cm]{figs/icons.png}
%     \caption{Respiratory audio and its application in healthcare scenarios.}
%     \label{fig:enter-label}
% \end{figure}
\section{Introduction}

% Why we should care about respiratory audio
Respiratory audio, such as coughing and breathing sounds generated by the respiratory system's airflow, captures multiple physiological characteristics of individuals and hence is useful for various health monitoring and disease detection applications~\cite{reichert2008analysis, sovijarvi2000definition}. For instance, audio recordings can be used to estimate respiratory rate and lung function~\cite{doheny2023estimation, rudraraju2020cough, xie2023earspiro}, detect snoring and apnea events during sleep~\cite{jane2000automatic, halevi2016can, romero2022acoustic}, assess the effect of smoking on health~\cite{ma2022determining, ma2023towards} and diagnose diseases like flu and asthma~\cite{jayadi2022embedded, islam2018multichannel,han2022sounds}.  
% Due to its easy-to-collect, non-invasive, and inexpensive nature, respiratory audio is crucial for sustainable healthcare. 


%However, despite its many advantages, respiratory audio remains under-explored within the machine learning community Compared to other health data modalities, as there are many generable for  clinical imaging [], electronic health records (EHRs) [], and medical time series [] 
%\jh{a summary and connect sentence is missing here?} 
%for feature extraction\jh{is feature learning better and boarder? I feel it is not just feature extraction as there is also feature selection, etc? }
 
To enable the wide adaption of these applications, high-performing algorithms are needed.
Most research relies on traditional signal processing methods~\cite{doheny2023estimation, rudraraju2020cough, jane2000automatic,halevi2016can, ma2022determining, jayadi2022embedded, islam2018multichannel}, which require domain knowledge and usually exhibit limited performance. Some deep acoustic models have been proposed~\cite{xie2023earspiro, han2022sounds,srivastava2021deep}, but since they are supervised, their performance heavily depends on the volume and quality of available labels, which are difficult and expensive to collect. Pretrained foundation models have a high potential to improve the performance of the models through transfer learning and supervised fine-tuning~\citep{dang2023human, xia2022exploring}. However, compared to other health data modalities like clinical imaging~\cite{pai2024foundation}, electronic health records (EHRs)~\cite{wornow2023shaky}, and medical time series~\cite{abbaspourazad2023large,dong2024simmtm}, foundation models for respiratory audio are largely under-explored. 
% \cm{We also argue}
% that for these models to be applied to sensitive healthcare applications they need to be first carefully examined~\cite{wu2024towards}.



\textbf{At present, there are no open-source pretrained respiratory acoustic foundation models}. 
Existing pretrained acoustic models like AudioMAE~\cite{huang2022masked} and CLAP~\cite{elizalde2023clap} are typically trained on general audio event datasets such as YouTube audio, containing very few respiratory sounds~\cite{jansen2017large, gemmeke2017audio} (e.g., only 0.3\% of the samples in Audioset~\cite{gemmeke2017audio} related to respiratory events). These models may not effectively capture the subtle nuances of respiratory sounds, which can vary in abrupt bursts, aperiodic components, and frequency distributions, particularly across different health conditions~\cite{reichert2008analysis}. Recently, a health acoustic representation model mainly pretrained on cough sounds has been presented~\cite{baur2024hear}; however, it is not open-source, making it hard to scrutinize its workings or compare. \tx{Added:} Recent years have witnessed an ever-increasing amount of respiratory audio being collected, particularly after the COVID-19 pandemic. However, no existing work has gathered and curated this data for training respiratory acoustic foundation models.
% d and is difficult to be widely used and fairly compared

\textbf{There is also a lack of ready-to-use benchmarks for respiratory audio research}\jh{these benchmarks is only for foundation models, can they be used for non-foundation model, can the scope be wider?} \tx{changed}. Current task-specific studies evaluate their models on their own datasets, leaving the models' generalizability to other tasks unclear~\cite{baur2024hear}. To facilitate the development of generalizable respiratory audio foundation models, a benchmark that combines multiple public datasets across diverse applications to enable fair and comprehensive evaluations is essential but currently lacking. 
This is particular crucial for safety-critical health applications, as models must be rigorously evaluated before use~\cite{wu2024towards,vollmer2020machine}.
% This is especially important in  trustworthy healthcare applications for models to be carefully examined before being applied.

%  challenge
%Most existing studies rely on traditional signal processing methods, which require domain knowledge and usually underperform. Although some deep learning methods have been developed, they require substantial labeled training data~\citep{dang2023human}. The challenge of data scarcity highlights the need for leveraging pretrained representation models to enhance the performance~\cite{}. To support diverse downstream applications, a desirable pretrained model must also be generalizable across tasks.

% One of the major challenges faced by respiratory audio based health applications is the scarcity of labelled data, which brings out the need for pretrained representation models to improve the performance. 

%  Although some deep learning methods have been developed, they are often tailored to and confined to a single task in training and evaluation.

% The need for 

% Although some deep learning methods have been developed, they are often confined to a single task in training and evaluation. These methods, tailored to specific tasks and constrained by limited data, may hinder generalization to new data and tasks.\yz{why pretrained model} In face of limited labelled data, pretrained representation models can be utilized to improve the performance.


% Most existing studies on respiratory audio health applications rely on traditional signal processing methods, which require domain knowledge and are usually under-performed.
% % This limitation is primarily due to the scarcity of data,
% Although some deep learning methods have been developed, they are often confined to a single task in training and evaluation. These methods, tailored to specific tasks and constrained by limited data, may hinder generalization to new data and tasks.\yz{why pretrained model} In face of limited labelled data, pretrained representation models can be utilized to improve the performance.
% %The main challenge in developing high-performing and generalizable models is the limited supervision caused by difficulties in acquiring health labels.
% %The problem is that the effectiveness of these task-specific models is often hindered by limited supervision due to difficulties in acquiring health labels. This remains a significant challenge for the widespread application of respiratory audio models. 

% In the broader field of computer audition,
% % particularly speech recognition, 
% many acoustic models have been pretrained using large-scale general audio datasets, such as audio from YouTube (so-called audio foundation models). These models could potentially serve as general feature extractors for health-related applications. However, we identify two unresolved issues:
% %\begin{itemize}[topsep=-1pt, itemsep=0pt, leftmargin=15pt]
% \textbf{1) There is a lack of open-source pretrained respiratory audio models}. Existing models are typically trained on speech corpora or audio event datasets []. They may not capture the subtle nuances of respiratory sounds, as respiratory audio can present various abrupt bursts, aperiodic components, and different frequency distributions [].
% \textbf{2) There is a lack of ready-to-use benchmarks for evaluating and comparing respiratory audio representation models}. Current task-specific studies evaluate their models on their own datasets, leaving the model generalizability unclear.
% % We anticipate that learning respiratory representation models is emerging, and a benchmark combining public datasets across diverse applications is urgently needed for fair and comprehensive evaluations.
% As the field of respiratory representation models is emerging, there is a clear need for a benchmark that combines public datasets across diverse applications to enable fair and comprehensive evaluations.
%\end{itemize}


 %\yz{The pergormance general audio pretrained models are unclear}.
 
% this paper, we provide a \underline{RE}s\underline{P}iratory \underline{A}ud\underline{I}o \underline{R}epresentation models learning and benchmarking \underline{S}ystem, named \textit{REPAIRS}, where we curate large-scale, multiple-source, public available respiratory health audio datasets,  to pretrain several models with different architectures and  SSL strategies, and compare them to existing general audio pretrained models on a wide number of applications.   [Adding a figure here?]

% reshape, respiratory health acoustic pretrained embedding
% restore
% rephase 

To mitigate these gaps, in this paper, we build \textit{OPERA}, an \textbf{OPE}n \textbf{R}espiratory \textbf{A}coustic foundation model pretraining and benchmarking system. It curates unlabeled respiratory audio datasets to pretrain foundation models and compares these models to existing pretrained acoustic models across various applications \yw{maybe point out the training mechanism more directly: It curated various unlabeled respiratory audio datasets to pretrain foundations and xxx?}.  Specifically,
\begin{itemize}[topsep=-1pt, itemsep=-1pt, leftmargin=15pt]
\item The respiratory audio datasets we curate for pretraining are large-scale (440 hours in total), multi-source (5 datasets), and publicly available (or available on request). They include breathing, coughing, and lung sounds acquired via both microphones and digital stethoscopes.
\item The foundation models we choose to pretrain consist of a lightweight CNN model and two state-of-the-art Transformers, and  two representative self-supervised learning strategies are used for their pretraining, i.e., contrastive and generative-based objectives.\jh{the two learning strategies * 3 models, make it sounds in total there are six? but in fact it is three. maybe the second half could be revised a bit, something like, and two representative self-supervised learning strategies were leveraged to pretrain these models, ie, contrastive and generative-based objectives?}. \yw{maybe we should add one sentence here to explain why we choose CNN and transformer? not only because they are sota, also they capture xxx features that suitable for audio signal?}
\item We also employ 10 labeled datasets (6 not covered by pretraining) to formulate 19 downstream evaluation tasks \yz{with linear evaluation}: 12 in health condition inference (classification) and 7 in lung function estimation (regression), to ensure fair, comprehensive and reproducible evaluation. \yw{fine-tune/linear evaluation the foundation evaluate on the downstream task? maybe add a bit more explaination about the evaluation modeling structure, as the previous sentence is talking about model structure.} \tx{we mainly use linear.}
\item We benchmark the performance of our 3 respiratory acoustic foundation models and 4 existing acoustic models on these downstream tasks as a start point for future exploration.  
\end{itemize}


% \tx{same model multi-tasks?}
Our extensive experiments reveal that our pretrained respiratory audio foundation models successfully encode valuable information on health conditions and respiratory indicators from the large-scale and heterogeneous respiratory-specific audio data, outperforming models that are not specifically pretrained on respiratory audio on 14 out of 19 tasks\yw{can we list a specific example here, e.g., compare with xxx existing model, our method encode xxx health conditions}. On health condition inference tasks, an AUROC (area under the receiver operating characteristic) score of over 0.7 is achieved in 6 tasks, yieiding comparable performance with existing literature. In lung function estimation, the respiratory audio foundation models demonstrate more stable performance across participants in addition to lower error in average, showing better generalizability and robustness which are crucial for healthcare. While these models yield promising results even with simple linear probing, fine-tuning them or using more complex architectures for prediction can further boost their performance. 
%Since these foundation models demonstrate generalizability across multiple downstream tasks, including new and unseen data sources and modalities, we move closer to a one-for-all target: training one model for all respiratory audio-driven applications~\cite{liu2023one}.
% \cm{more on findings?}
\yz{more on findings}

These foundation models demonstrate generalizability across multiple downstream tasks, including new and unseen data sources and modalities, getting one important step closer to a single model with effective use on a large range of respiratory audio applications ~\cite{liu2023one}.\cm{i changed this sentence, not sure about this citation: is it suitable? i find it weird we have a citation here as it decreases our novelty. we say we move the community closer to one model fitting all but then we cite someone else?}




%This advancement is one step towards general intelligence for health acoustic modelling. 


% Consistent with previous findings~\cite{liu2021self}, we observed that contrastive pretraining benefits classification tasks more, while the generative pretrained models perform better on regression tasks. It is also interesting to see that a light-weight CNN model achieves a good trade-off between efficiency and performance.

% \cm{talk about implications of this on health applications? or large scale applicabillity?}

In summary, this paper provides \textit{the first open-sourced respiratory acoustic foundation model pretraining and benchmarking system}. This represents a critical first step towards %\cm{explainable}\tx{emm, we are not explainable yet} 
comprehensive and reproducible audio foundation models for health. It will facilitate progress in both the healthcare and machine learning communities to develop and evaluate their work. These efforts will extend current machine learning capabilities, now able to \textit{see} (via vision) and \textit{read} (via natural languages), to also \textit{listen} (via audio) to our health.

%Respiratory diseases are a leading cause of morbidity and mortality worldwide. Early diagnosis and screening are crucial for effective treatment and improved patient outcomes. Recently, there has been growing interest in leveraging respiratory sounds, such as breathing and coughing, as non-invasive sources of diagnostic information~\cite{dang2023human}. They can be easily collected from mobile devices and provide valuable insights into the physiological state of the respiratory system.


%Deep learning models have emerged as powerful tools for modelling respiratory sounds. However, their effectiveness is often hindered by the limited availability of labeled data for respiratory condition classification. Recent advances in generative AI demonstrate the potential for large-scale pretraining to enhance performance across various tasks~\cite{krishnan2022self}, but there is currently a lack of open pretrained models specifically tailored to respiratory audio data. Existing models, typically trained on large image datasets or general-purpose audio data, may lack the necessary domain-specific knowledge to capture the subtle nuances of respiratory sounds.
% Consequently, their performance on respiratory disease classification tasks suffers unless they are further fine-tuned with a substantial amount of labeled respiratory data, which is scarce and expensive to acquire.

%By providing a pretrained model tailored specifically to respiratory sounds, we aim to address the challenge of data scarcity in downstream tasks and offer a valuable resource for the field of respiratory disease diagnosis and screening. Such a model has the potential to empower researchers and developers to build more robust and accurate models for early disease detection. 





==> sections/04application_old.tex <==
\vspace{-5pt}
\section{Benchmarking}\label{sec:benchmark}
\vspace{-5pt}
\subsection{Benchmark Datasets and Tasks Setup}
\vspace{-5pt}
% This work introduces a new benchmark for evaluating respiratory audio foundation models, the 19 tasks are summraized in \cref{tab:task}. \yz{here or 5.1?} \tx{blew is better}
\input{tables/downstream-task}

\textbf{Tasks}. 
To facilitate the evaluation of our pretrained models, existing acoustic representation models, and future emerging respiratory acoustic foundation models, we introduce a new benchmark. A total of 10 labeled respiratory audio datasets, encompassing 6 respiratory audio modalities, are curated for this benchmark. Among these 10 datasets, 6 are new and unseen during the pretraining stage.

Using these 10 datasets, we formulate 19 downstream tasks, including 12 health condition inference tasks and 7 lung function estimation tasks. The health condition inference tasks cover disease detection such as COVID-19 and COPD (Chronic Obstructive Pulmonary Disease),
% \cm{spell out?}), 
participant attribute inference (e.g., smoker, gender), disease severity classification, and body position in sleep monitoring. These are classification tasks. Tasks 1 to 10 are binary, while Tasks 11 and 12 have 5 classes. The lung function estimation tasks include spirometry test performance estimation and respiratory rate estimation. These are regression tasks aimed at predicting continuous values.
Data and task statistics are summarized in \cref{tab:task}, with detailed descriptions provided in the Appendix. 



\textit{All data in this benchmark are publicly available or under controlled access procedures} %can be easily accessed upon request for research purposes} 
(licenses are detailed in Appendix). When available, we follow the official train-test split (Tasks 1-4 and 12-18); otherwise, we implement a random participant-independent split to ensure realistic evaluation (Tasks 5-11 and 19). Due to the limited number of participants in Tasks 13-19, we employ leave-one-(participant)-out evaluation. For all other tasks, we adopt a fixed train-validation-test split.
% For these tasks, we report the standard deviation across participants. 
% For all other tasks, we adopt a fixed train-validation-test split and report the standard deviation obtained from five independent experiments using different model initializations.

\textbf{Baselines}. In addition to our pretrained models, we also include a commonly used acoustic feature set and three open pretrained acoustic models in this benchmark. They are \textbf{Opensmile} ~\cite{eyben2010opensmile} (\textit{Emobase} acoutic feature set), \textbf{VGGish}~\cite{hershey2017cnn} (supervised pretrained), \textbf{AudioMAE}~\cite{huang2022masked} (self-supervised pretrained) and \textbf{CLAP}~\cite{elizalde2023clap} (language-supervised pretrained). We consider these four methods as baselines to be distinguished from our pretrained models.

\textbf{Evaluation protocol}. All tasks are evaluated using the standard linear probe protocol~\cite{chen2020simple, saeed2021contrastive, niizumi2021byol}: training a single fully connected layer on top of the representations extracted from the frozen encoder. Linear evaluation focuses on the quality of learned representations and is applicable for some very small datasets. 
%Additional evaluation methods, such as fine-tuning and temporal dynamics modelling, will be discussed in \cref{sec:discussion}. 
\textbf{AUROC} (area under the receiver operating characteristic) is reported for classification (Task 1-12) and \textbf{MAE} (mean absolute error) is reported for regression (Task 13-19). For a comprehensive overall evaluation, we report \textbf{MRR} (mean reciprocal rank) across tasks~\cite{shi2012climf}). 
% \jh{MRR is not introduced here?} \yz{added}

For baselines, both the data pre-processing and feature extraction strictly follow their official implementation. For our pretrained models, the same audio preprocessing is used as in pretraining. OPERA-CT and OPERA-CE require minimum input audio lengths of 8 seconds and 2 seconds, respectively. Therefore, for recordings shorter than these lengths, padding is applied to extend the audio (repeat padding is applied for Tasks 1-12 and zero padding for Tasks 13-19, according to the task properties)~\cite{hershey2017cnn, elizalde2023clap}. OPERA-GT has a maximum input length of 8 seconds. For recordings exceeding 8 seconds, they are segmented into frames of up to 8 seconds, and we use the averaged representation over these frames as the input for the linear layer~\cite{huang2022masked}.
\textit{Note that 
%all the evaluations for 
the baselines and our pretrained models are implemented within the same pipeline, %in our system, 
making our results easy to reproduce and our benchmark ready to use.}



% When an audio recording is shorter than model input, repeat padding is applied for Task 1-12 and zero padding for Task 13-19, according to the task properties. 
% When the length of a recording exceeds the model's maximum input length (for , OPERA-GT )

% When the sample is too long, we segment the audio and average the feature following common practice~\cite{hershey2017cnn, xia2022exploring, elizalde2023clap}.


% we preprocess the audio of each tasks to match default input format before feature extraction, including clipping, segmentation and calculation of spectrogram or filter bank features. For our pretrained models, we use the same spectrogram preprocessing as in pretraining. When the audio sample is not long enough for model input, we adopt repeat padding for the classification tasks and zero padding for regression tasks. When the sample is too long, we segment the audio and average the feature following common practice~\cite{hershey2017cnn, xia2022exploring, elizalde2023clap}. \yz{should we mention somethere that our model has less constraint on input audio length, maybe discussion and future work?}
% \tx{this is not only 'pre-process', once the length exceeds the window, we also average the features. Need to better introduce this.}


\input{tables/rank}
\begin{figure*}[t]
    \centering
    \subfigure[Health Condition Inference]{\includegraphics[height=5.5cm]{figs/radarRank_health.png} \label{fig:radar:health}}
    \subfigure[Lung Function Estimation]{ \includegraphics[height=5.5cm]{figs/radarRank_lung.png} \label{fig:radar:lung}}
     \setlength{\abovecaptionskip}{0.1cm}
    \caption{Radar plot of reciprocal ranks on two groups of tasks.
    % \jh{is it common to use radar plot on the RR measures? even second is quite far from the first. Why the tasks are not in order, by purpose?}\yz{for better visualization purpose..}
    }
    \label{fig:radar}
    \vspace{-15pt}
\end{figure*}

\subsection{Experimental Results} 

% \tx{better: compared 4 baseline}
\textbf{Overall performance. }
Across the 19 tasks on 10 datasets, our experimental results show that OPERA-CT performs the best, followed by OPERA-GT, as measured by their mean reciprocal rank of 0.5576 and 0.4947 (see \cref{tab:rank}). The reciprocal ranks of all evaluated methods are detailed in \cref{fig:radar}, with the performance metrics for each task summarized in \cref{tab:res:health} and \cref{tab:res:lung}.


From \cref{tab:rank}, it is evident that our pretrained respiratory  acoustic foundation models  outperforms the four general audio feature set and pretrained representations. This advantage likely stems from the exposure to large-scale and heterogeneous respiratory-specific audio data. 
% \cm{this is something to say in abstract and intro!}
Specifically, OPERA-CT performs the best in 7 out of the 12 health condition inference tasks (see \cref{fig:radar:health}, with a mean reciprocal rank as high as 0.7361 (see \cref{tab:rank}). For lung function estimation tasks, OPERA-GT performs the best in 3 out of the 7 tasks  (see \cref{fig:radar:lung}, with a mean reciprocal rank of 0.5714 (see \cref{tab:rank}). This suggests a strong representation ability of the transformer architecture for audio.  As a lightweight CNN model, OPERA-CE also demonstrate satisfactory results, with a mean reciprocal of 0.4690 and performs second best in lung function estimation tasks (see \cref{tab:rank}).




%\tx{Work: encoding useful information, compared to reference if possible}
\textbf{Task-specific performance.} 
Looking into the task performance measured by AUROC or MAE, there are some insightful observations.  First of all, our implementation of the seven methods yield comparable performance with those reported in the literature.
% \cm{another finding for the intro?}
For example, cough-based COVID-19 detection as reported can achieve an AUROC about 0.65~\cite{coppock2024audio, xia2021covid}, and Task 2 in our benchmark yields an average AUROC of 0.640. This demonstrates the reliability of our benchmark and promise of respiratory audio foundation models for health. 

In terms of the classification performance,
% for the health condition inference tasks,
an AUROC exceeding 0.7 is generally considered desirable to demonstrate the utility of the extracted features~\cite{fawcett2006introduction}. As shown in \cref{tab:res:health}, among the 12 health condition inference tasks, our pretrained OPERA models achieve AUROC exceeding 0.7 on 6 tasks (Task 2, 6, 7, 9, 10, and 12), while the best baseline CLAP only surpasses this threshold on 4 tasks (Task  7, 9, 10, and 12). This indicates that our pretrained models can better encode health condition-related information from the respiratory audio. 
% compared to the baseline models.
% \cm{another finding?}
We also note that all models exhibited higher AUROC for tasks involving demographic factors (Task 6 and 9) than disease detection (Task 1, 2, 5, 7, 10, and 11). This observation implies that subtle pathological differences in respiratory audio signatures might be more challenging to detect than demographic variations, necessitating more powerful models for accurate capture. %Nevertheless, even within this context, our OPERA models demonstrate superior performance compared to the baselines. 
We recognize the limited AUROC (0.6$\sim$ 0.8) reported in this benchmark, and we also encourage more future studies to improve the metric for those tasks. 




Regarding the regression performance for the lung function estimation, those tasks require the model to be able to capture the global dynamics from the entire audio sample and the lower the MAE, the better the performance. 
% Our pretrained models reduce the error in FEV1 estimation using breathing sounds (Task 2) from  0.859 (Opensmile)  to 0.771 (OPERA-CE), FVC estimation using vowel sounds (Task 4) from 0.710 (CLAP) to 0.593 (OPERA-GT), FEV1 estimation using vowel sounds (Task 5) from 0.605 (Opensmile) to 0.561 (OPERA-GT), and respiratory rate estimation (Task 19) from 2.611 (VGGish) to 2.537 (OPERA-GT). 
Our pretrained models reduce the error in FEV1 estimation using breathing sounds (Task 14), FVC estimation using vowel sounds (Task 16), FEV1 estimation using vowel sounds (Task 17), and respiratory rate estimation (Task 19). 
Not only a lower MAE, but also a smaller standard deviation across subjects are archived. Since Task 13-19 use leave-one(subject)-out cross validation, the models usually represent a high variance given the difference among subjects. A small standard deviation
% \cm{spell out}
suggest that our representations are more generalizable and robust to different subjects, which are of great importance for healthcare applications. \textcolor{red}{Can you explain why OPERA models did not work well mainly on regression tasks wrt baseline models for tasks 13, 15 and 18} 
% \cm{another finding}
 

\input{tables/downstream-health}
\input{tables/downstream-lung}

\textbf{Other findings.}
From \cref{tab:rank}, \cref{tab:res:health} and \cref{tab:res:lung}, it can also be observed that the models pretrained with a contrastive objective (OPERA-CT, OPERA-C) generally achieve superior performance on classification tasks (i.e., health condition inference),  while the generative pretrained models ( AudioMAE and OPERA-GT) perform better on regression tasks (i.e., lung function estimation). This aligns with the inherent nature of the methods, as contrastive learning’s discriminative training goal naturally aligns with the classification objective, and it discards the decoder in the architecture compared to generative models.
% \jh{one question, why not combine the two training strategies?}\yz{combing the two}
This finding is consistent with prior observations from~\cite{liu2021self} on various vision benchmarks.
Besides, our models demonstrate good generalization capabilities to unseen datasets (Task 8-19) and unseen respiratory audio modalities including snoring sounds (Task 12) and vowel sounds (Tasks 16-18) which are not used for pretraining. 
% \tx{What do we want to say here?}

%compared to the literature or the linear evlation.... 


% contrastive learning’s goal naturally conforms the classification objective,
% Because contrastive learning has assumed the downstream applications to be classifications, it only employs the encoder and discards the decoder in the architecture compared to generative models. Therefore, contrastive models are usually light-weighted and perform better in discriminative downstream applications.



%Within the contrastive models, the lightweight EfficientNet-based OPERA-CE offers a smaller size and improved efficiency at the expense of a slight performance trade-off. Despite its size of only 4 million parameters, OPERA-CE surpasses baseline models (VGGish: 62M, AudioMAE: 86M, CLAP: 80M),  and maintains a good balance between classification and regression tasks.
%\yz{don't know why though (justification for this observation might be explored in future work?).}

% \textbf{Health Condition Inference Performance}. \cref{tab:res:health} shows the performance of various inference tasks. Disease detection and severity classification present inherent challenges, as reflected in their lower scores compared to tasks like gender identification (Tasks 6 and 9). Pretraining on respiratory audio improves performance across the tasks. It is worth noting that our contrastive-based models generalize well to new modalities unseen during OPERA training, such as snoring, even outperforming baselines trained with snoring data included (VGGish, AudioMAE and CLAP). 
% This suggests that contrastive training specifically on respiratory data helps the model distinguish nuances between these sounds, applicable to new modalities as well. Among the baselines, CLAP achieves strong results due to its exposure to a large-scale and diverse training dataset – unlike VGGish and AudioMAE, which solely rely on AudioSet.

% \textbf{Lung Function Estimation Performance}. These tasks are challenging for all models using linear regression, probably due to the very limited number subject to train generalable regression model. Opensmile feature set proves a strong baseline in this setting. \yz{}


% \input{tables/participant}
% \subsection{Category 1}

% \input{tables/event-level}
% \subsection{Category 2}

% \input{tables/lungfunction}

% \subsection{Category 2}

==> sections/app05code.tex <==
\subsection{Usage}

% \begin{verbatim}
% \colorbox{mygrey}{
%   function sum(a, b) {
%     return a + b;
%   }
%   }
% \end{verbatim}


% \begin{lstlisting}
% Adjust color name or RGB values
% def sum(a, b):
%   """Returns the sum of a and b."""
%   return a + b
% \end{lstlisting}

\begin{python}
# A comment
x = [5, 7, 10]
y = 0

for num in x:
    y += num
    
print(y)
\end{python}

==> tables/demographic_table.tex <==
% \usepackage{color}
% \usepackage{tabularray}
\begin{table}[t]
\caption{Downstream task characteristics grouped by task category. Datasets in grey are entirely new (not used in pretraining), while others have test sets held out unseen. For T13-T19, FVC denotes forced vital capacity (L), FEV1 is the forced expiratory volume in 1 second, and FEV1/FVC refers to the ratio of the two. 
% For T19, 1297 samples are from 16 subjects. 
% \jh{how many subjects in MMlung, it is not given? will it be good to list #subjects in the table?} 
% \yz{adding \# subjects}
}
\centering
\begin{adjustbox}{width=\textwidth,center} % {width=\columnwidth,center}
\begin{tabular}{rlllllllll}
 
% \Large \textbf{Health condition inference} \\
% \toprule
\toprule
\textbf{Dataset} & \textbf{ID}    & \textbf{Task}             & \textbf{Modality} & \textbf{\#Sam. (\#Sub.)} & \textbf{Data Distribution} \\
% \textbf{train} & \textbf{val}  & \textbf{test}          &         
 % \textbf{Ref}           \\
\midrule
\textbf{UK~COVID-19}~\cite{coppock2024audio}      & T1 & Covid / Non-covid         & Exhalation             & 2500  (2500)        & 840 / 1660                         \\
                         & T2 & Covid / Non-covid           & Cough             & 2500  (2500)        & 840 / 1660                         \\
\textbf{COVID-19 Sounds}~\cite{xia2021covid}   & T3 & Symptomatic / Healthy       & Breath             & 4138 (3294)        & 2029 / 2109                    \\
                         & T4 & Symptomatic / Healthy       & Cough             & 4138 (3294)       & 2029 / 2109                           \\
\textbf{CoughVID}~\cite{orlandic2021coughvid}         & T5 & Covid / Non-covid           & Cough             & 6175  (n/a)       & 547 / 5628                             \\
                         & T6 & Female / Male               & Cough             & 7263 (n/a)       & 2468 / 4795                            \\
\textbf{ICBHI}~\cite{rocha2019open}           & T7 & COPD / Healthy              & Lung sounds             & 828 (90)        & 793 / 35             \\
%\colorrow
\textbf{Coswara}~\cite{bhattacharya2023coswara}          & T8 & Smoker / Non-smoker         & Cough             & 948  (n/a)        & 201 / 747                              \\
%\colorrow
                         & T9 & Female / Male               & Cough             & 2496  (n/a)       & 759 / 1737                  \\
  %\colorrow
\textbf{KAUH}~\cite{fraiwan2021dataset}           & T10 & Obstructive / Healthy       & Lung sounds             & 234 (79)        & 129 / 105                  \\
%\colorrow
\textbf{Respiratory@TR}~\cite{altan2017multimedia}                & T11 & COPD severity             & Lung sounds            & 504 (42)        & 72 / 60 / 84 / 84 / 204                   \\
%\colorrow
\textbf{SSBPR}~\cite{xiao2023snoring}           & T12 & Body position recognition & Snoring             & 7468 (20)       & 1638 / 1454 / 1269 / 1668 / 1439             \\


\midrule


% \\
% \Large \textbf{Lung function estimation} \\
% \toprule
% \textbf{Dataset} & \textbf{Task}             & \textbf{Mod.} & \textbf{\#} & \textbf{data distribution} &


% \textbf{train} & \textbf{val}  & \textbf{test}          &         
 % \textbf{Ref}           \\
% \toprule

%\colorrow
\textbf{MMlung}~\cite{mosuilymmlung}           & T13 & FVC                       & Deep breath          & 40 (40)         & 3.402 ± 1.032 L                    \\
%\colorrow
                         & T14 & FEV1                      & Deep breath           & 40   (40)          & 2.657 ± 0.976 L                  \\
  %\colorrow
                         & T15 & FEV1/FVC                  & Deep breath             & 40   (40)          & 0.808 ± 0.190 L                       \\
   %\colorrow
                         & T16 & FVC                       & O   Vowels         & 40   (40)          & 3.402 ± 1.032 L                \\
    %\colorrow
                         & T17 & FEV1                      & O   Vowels              & 40    (40)         & 2.657 ± 0.976 L                         \\
    %\colorrow
                         & T18 & FEV1/FVC                  & O   Vowels               & 40   (40)          & 0.808 ± 0.190 L                  \\
    %\colorrow
\textbf{NoseMic}~\cite{butkow2024evaluation}          & T19 & Respiratory rate          & Breath             & 1297 (16)     & 13.915 ± 3.386 bpm                   \\


  \bottomrule     
\end{tabular}
% Performance on health status inference tasks.
\end{adjustbox}
\label{tab:task}
\end{table}

==> tables/downstream-health-significance.tex <==




% \usepackage{color}
% \usepackage{tabularray}
\begin{table}[t]
\caption{AUROC on health condition inference tasks (\textcolor{red}{higher} is better).  The best model for each task is highlighted. We report mean and standard deviation from five independent runs. \textcolor{red}{\checkmark} and \textcolor{red}{*} indicates superiority over the opensmile feature set and the other pretrained baselines respectively.\yz{T5, T6 and T10 updated. T11}
% \tx{We need to label the best baseline I think}
% \jh{do you also want to highlight the second best here?}
% \yz{not highlighting it looks better for us}\jh{it is not very clear to me what are the std, is the evaluation on multiple runs, apart from some used leave-one-out?} \yz{added}
}
%$\Delta$ shows the relative improvement of the best respiratory audio foundation model over the baselines.}
\centering
\begin{adjustbox}{width=0.99\textwidth,center} % {width=\columnwidth,center}
\begin{tabular}{ll|c|ccc|ccc|c}
\toprule
ID & Task Abbr.        & Opensmile     & VGGish        & AudioMAE      & CLAP                                                                    & \textbf{OPERA-CT}  &                                                \textbf{OPERA-CE}                                 & \textbf{OPERA-GT}                  &                                            \\ 
\midrule

T1      & Covid (Exhale)    & 0.550 ± 0.015 & 0.573 ± 0.004 & 0.549 ± 0.001 & 0.547 ± 0.003                                                           & \cellcolor{mypink}{}0.588 ± 0.002$\dagger$                                                          & 0.557 ± 0.003 $\dagger$                  & {0.577 ± 0.007~~} &\textcolor{red}{\checkmark*} \\
T2      & Covid (Cough)     & 0.623 ± 0.028 & 0.557 ± 0.005 & 0.616 ± 0.001 & 0.627 ± 0.003                                                           & \cellcolor{mypink}{0.701 ± 0.002$\dagger$}& 0.629 ± 0.006~~                                                           & 0.677 ± 0.001$\dagger$                                &\textcolor{red}{\checkmark*}                            \\
T3      & Symptom (Breath) & 0.571 ± 0.006 & 0.571 ± 0.003 & 0.583 ± 0.003 & 0.611 ± 0.006                                                           & 0.603 ± 0.005$\dagger$                                                            & 0.615 ± 0.005~~                    & \cellcolor{mypink}{0.615 ± 0.002~~}  &\textcolor{red}{\checkmark*}\\
T4      & Symptom (Cough)  & 0.633 ± 0.012 & 0.605 ± 0.004 & 0.659 ± 0.001 & 0.674 ± 0.001                                                           & \cellcolor{mypink}{0.681 ± 0.006~~}& 0.664 ± 0.001$\dagger$                                                            & 0.670 ± 0.002$\dagger$                                   &\textcolor{red}{\checkmark*}                          \\
% T5      & Covid (Cough)    & 0.546 ± 0.008 & 0.602 ± 0.001 & 0.549 ± 0.005 & 0.603 ± 0.013                                                           & \cellcolor{mypink}{0.609 ± 0.004}& 0.584 ± 0.003                                                           & 0.575 ± 0.006                                   &\textcolor{red}{\checkmark*}                    \\
% T6      & Gender (Cough)   & 0.639 ± 0.010 & 0.608 ± 0.000 & 0.666 ± 0.002 & 0.684 ± 0.002                                                           & \cellcolor{mypink}{0.801 ± 0.000}& 0.722 ± 0.004                                                           & 0.762 ± 0.001                                     &\textcolor{red}{\checkmark*}                       \\
T5      & Covid (Cough)   & 0.537 ± 0.011	 & 0.538 ± 0.028  & 	0.554 ± 0.004 & 	\cellcolor{mypink}{}0.599 ± 0.007	 & 0.578 ± 0.001$\dagger$	 & 0.566 ± 0.008$\dagger$	 & 0.552 ± 0.003$\dagger$ & \textcolor{red}{\checkmark~~}  \\
T6      & Gender (Cough)   & 0.677 ± 0.005	 & 0.600 ± 0.001  & 	0.628 ± 0.001	 & 0.665 ± 0.001 & 	\cellcolor{mypink}{}0.795 ± 0.001$\dagger$	 & 0.721 ± 0.001$\dagger$	 & 0.735 ± 0.000$\dagger$ & \textcolor{red}{\checkmark*}   \\

T7      & COPD (Lung)        & 0.579 ± 0.043 & 0.605 ± 0.077 & 0.886 ± 0.017 & \cellcolor{mypink}{0.933 ± 0.005}& 0.855 ± 0.012$\dagger$                                                           & 0.872 ± 0.011$\dagger$                                                           & 0.741 ± 0.011$\dagger$                                     &\textcolor{red}{\checkmark}~~                       \\
T8      & Smoker (Cough)   & 0.534 ± 0.060 & 0.507 ± 0.027 & 0.549 ± 0.022 & 0.676 ± 0.004                                                           & \cellcolor{mypink}{0.685 ± 0.012~~}& 0.674 ± 0.013~~                                                           & 0.650 ± 0.005$\dagger$                                       &\textcolor{red}{\checkmark*}                     \\
T9      & Gender (Cough)     & 0.753 ± 0.008 & 0.606 ± 0.003 & 0.724 ± 0.001 & 0.742 ± 0.001                                                           & \cellcolor{mypink}{0.874 ± 0.000$\dagger$ }& 0.801 ± 0.002$\dagger$                                                            & 0.825 ± 0.001$\dagger$                                        &\textcolor{red}{\checkmark*}                     \\
% T10     & Obstructive (Lung)            & 0.502 ± 0.080 & 0.505 ± 0.110 & 0.614 ± 0.040 & 0.703 ± 0.036                                                           & 0.719 ± 0.018                                                           & \cellcolor{mypink}{0.742 ± 0.014}& 0.700 ± 0.013                            &\textcolor{red}{\checkmark*}                                \\
T10     & Obstructive (Lung)            & 0.636 ± 0.082 &	0.605 ± 0.036 &		0.616 ± 0.041 &		0.697 ± 0.004	&	0.722 ± 0.016$\dagger$	&	\cellcolor{mypink}0.741 ± 0.014$\dagger$	&	0.703 ± 0.016~~ &\textcolor{red}{\checkmark*}  \\
T11     & COPD severity (Lung)     & 0.494 ± 0.054 & 0.590 ± 0.034 & 0.510 ± 0.021 & 0.636 ± 0.045                                                           & 0.625 ± 0.038~~                                                           & \cellcolor{mypink}{0.683 ± 0.007$\dagger$}& 0.606 ± 0.015~~                                  &\textcolor{red}{\checkmark*}                          \\
T12     & Position (Snoring)       & 0.772 ± 0.005 & 0.657 ± 0.002 & 0.649 ± 0.001 & 0.702 ± 0.001                                                           & \cellcolor{mypink}{0.781 ± 0.000$\dagger$}& 0.769 ± 0.000~~                                                           & 0.742 ± 0.001$\dagger$                               &\textcolor{red}{\checkmark*}                          \\


% Task  & Opensmile     & VGGish        & AudioMAE      & CLAP      & \textbf{OPERA-CT} & \textbf{OPERA-CE} & \textbf{OPERA-GT} \\
% \midrule

% T1   & 0.550 ± 0.015   & 0.580 ± 0.001 & 0.549 ± 0.001 & 0.565 ± 0.001 & 0.586 ± 0.008   & 0.551 ± 0.010   & \cellcolor{mypink}{0.605 ± 0.001}   \\
% T2   & 0.649 ± 0.006 & 0.557 ± 0.005 & 0.616 ± 0.001 & 0.648 ± 0.003 & \cellcolor{mypink}{0.701 ± 0.002}   & 0.629 ± 0.006   & 0.677 ± 0.001   \\
% T3   & 0.571 ± 0.006 & 0.571 ± 0.003 & 0.583 ± 0.003 & 0.611 ± 0.006 & 0.603 ± 0.005   & 0.610 ± 0.004   & \cellcolor{mypink}{0.613 ± 0.002}   \\
% T4   & 0.633 ± 0.012 & 0.605 ± 0.004 & 0.659 ± 0.001 & 0.669 ± 0.002 & \cellcolor{mypink}{0.680 ± 0.006}   & 0.665 ± 0.001   & 0.673 ± 0.001   \\
% T5   & 0.546 ± 0.008 & 0.602 ± 0.001 & 0.549 ± 0.005 & 0.603 ± 0.013 & \cellcolor{mypink}{0.609 ± 0.004}   & 0.584 ± 0.003   & 0.575 ± 0.006   \\
% T6   & 0.639 ± 0.010 & 0.608 ± 0.000 & 0.666 ± 0.002 & 0.684 ± 0.002 & \cellcolor{mypink}{0.801 ± 0.000}   & 0.722 ± 0.004   & 0.762 ± 0.001   \\
% T7   & 0.579 ± 0.043 & 0.605 ± 0.077 & 0.886 ± 0.017 & \cellcolor{mypink}{0.933 ± 0.005} & 0.855 ± 0.012   & 0.872 ± 0.011   & 0.741 ± 0.011   \\
% T8   & 0.534 ± 0.060  & 0.507 ± 0.027 & 0.549 ± 0.022 & 0.680 ± 0.009 & \cellcolor{mypink}{0.685 ± 0.012}   & 0.674 ± 0.013   & 0.650 ± 0.005   \\
% T9   & 0.753 ± 0.008 & 0.606 ± 0.003 & 0.724 ± 0.001 & 0.742 ± 0.001 & \cellcolor{mypink}{0.874 ± 0.000}   & 0.801 ± 0.002   & 0.825 ± 0.001   \\
% T10  & 0.502 ± 0.080  & 0.505 ± 0.110  & 0.614 ± 0.040 & 0.703 ± 0.036 & 0.719 ± 0.018   & \cellcolor{mypink}{0.742 ± 0.014}   & 0.700 ± 0.013   \\
% T11  & 0.494 ± 0.054 & 0.590 ± 0.034 & 0.510 ± 0.021 & 0.635 ± 0.040 & 0.625 ± 0.038   & \cellcolor{mypink}{0.683 ± 0.007}   & 0.615 ± 0.019   \\
% T12  & 0.772 ± 0.005 & 0.657 ± 0.002 & 0.649 ± 0.001 & 0.702 ± 0.001 & \cellcolor{mypink}{0.781 ± 0.000}   & 0.769 ± 0.000   & 0.742 ± 0.001   \\

% T1   & 0.550 ± 0.015   & 0.580 ± 0.001 & 0.549 ± 0.001 & 0.565 ± 0.001 & \cellcolor{myblue}0.586 ± 0.008   & 0.551 ± 0.010   & \cellcolor{mypink}{0.605 ± 0.001}   \\
% T2   & 0.649 ± 0.006 & 0.557 ± 0.005 & 0.616 ± 0.001 & 0.648 ± 0.003 & \cellcolor{mypink}{0.701 ± 0.002}   & 0.629 ± 0.006   & \cellcolor{myblue}0.677 ± 0.001   \\
% T3   & 0.571 ± 0.006 & 0.571 ± 0.003 & 0.583 ± 0.003 & \cellcolor{myblue}0.611 ± 0.006 & 0.603 ± 0.005   & 0.610 ± 0.004   & \cellcolor{mypink}{0.613 ± 0.002}   \\
% T4   & 0.633 ± 0.012 & 0.605 ± 0.004 & 0.659 ± 0.001 & 0.669 ± 0.002 & \cellcolor{mypink}{0.680 ± 0.006}   & 0.665 ± 0.001   & \cellcolor{myblue}0.673 ± 0.001   \\
% T5   & 0.546 ± 0.008 & 0.602 ± 0.001 & 0.549 ± 0.005 & \cellcolor{myblue}0.603 ± 0.013 & \cellcolor{mypink}{0.609 ± 0.004}   & 0.584 ± 0.003   & 0.575 ± 0.006   \\
% T6   & 0.639 ± 0.010 & 0.608 ± 0.000 & 0.666 ± 0.002 & 0.684 ± 0.002 & \cellcolor{mypink}{0.801 ± 0.000}   & 0.722 ± 0.004   & \cellcolor{myblue}0.762 ± 0.001   \\
% T7   & 0.579 ± 0.043 & 0.605 ± 0.077 & \cellcolor{myblue}0.886 ± 0.017 & \cellcolor{mypink}{0.933 ± 0.005} & 0.855 ± 0.012   & 0.872 ± 0.011   & 0.741 ± 0.011   \\
% T8   & 0.534 ± 0.060  & 0.507 ± 0.027 & 0.549 ± 0.022 & \cellcolor{myblue}0.680 ± 0.009 & \cellcolor{mypink}{0.685 ± 0.012}   & 0.674 ± 0.013   & 0.650 ± 0.005   \\
% T9   & 0.753 ± 0.008 & 0.606 ± 0.003 & 0.724 ± 0.001 & 0.742 ± 0.001 & \cellcolor{mypink}{0.874 ± 0.000}   & 0.801 ± 0.002   & \cellcolor{myblue}0.825 ± 0.001   \\
% T10  & 0.502 ± 0.080  & 0.505 ± 0.110  & 0.614 ± 0.040 & 0.703 ± 0.036 & \cellcolor{myblue}0.719 ± 0.018   & \cellcolor{mypink}{0.742 ± 0.014}   & 0.700 ± 0.013   \\
% T11  & 0.494 ± 0.054 & 0.590 ± 0.034 & 0.510 ± 0.021 & \cellcolor{myblue}0.635 ± 0.040 & 0.625 ± 0.038   & \cellcolor{mypink}{0.683 ± 0.007}   & 0.615 ± 0.019   \\
% T12  & 0.772 ± 0.005 & 0.657 ± 0.002 & 0.649 ± 0.001 & 0.702 ± 0.001 & \cellcolor{mypink}{0.781 ± 0.000}   & \cellcolor{myblue}0.769 ± 0.000   & 0.742 ± 0.001   \\

  \bottomrule     
\end{tabular}
% Performance on health status inference tasks.
\end{adjustbox}
\label{tab:res:health}
\vspace{-5pt}
\end{table}



% | Task                       | Opensmile     | VGGish       | AudioMAE      | CLAP  | **OPERA-CT** |     **OPERA-CE**  |**OPERA-GT**   |
% | ---------------------------| ---------| ---------| ---------| ---------| ---------| ---------|---------|
% |T11  COPD severity (Lung)   | 0.494 ± 0.054 | 0.590 ± 0.034 | 0.510 ± 0.021 | 0.636 ± 0.045   | 0.625 ± 0.038 | **0.683 ± 0.007** |0.606 ± 0.015   |   

==> tables/downstream-lung-significance.tex <==

\begin{table}[t]
\caption{MAE on lung function estimation tasks (\textcolor{red}{lower} is better). Best model per task is highlighted. We report mean and standard deviation across subjects. }
\centering
\begin{adjustbox}{width=0.99\textwidth,center} % {width=\columnwidth,center}
\begin{tabular}{ll|c|ccc|cccccc|c}
\toprule
ID & Task Abbr.  & Opensmile     & VGGish        & AudioMAE      & CLAP          & \textbf{OPERA-CT} & \textbf{OPERA-CE} & \textbf{OPERA-GT} &\\
  \midrule
T13 & FVC (Breath)          &0.985 ± 0.743	&0.904 ± 0.568	&0.900 ± 0.551	&0.896 ± 0.542	&0.924 ± 0.583	&\cellcolor{mypink}0.848 ± 0.607	&0.892 ± 0.618 &\textcolor{red}{\checkmark*}\\
T14 & FEV1 (Breath)         & \cellcolor{mypink}0.756 ± 0.721	&0.839 ± 0.563	&0.821 ± 0.590	&0.840 ± 0.547	&0.837 ± 0.563	&0.834 ± 0.581	&0.825 ± 0.560 &  \\
T15 & FEV1/FVC (Breath)     & 0.141 ± 0.185	&0.131 ± 0.146	&0.129 ± 0.146	&0.134 ± 0.146	&\cellcolor{mypink}0.128 ± 0.140	&0.132 ± 0.141	&\cellcolor{mypink}0.128 ± 0.141 &\textcolor{red}{\checkmark*}\\
T16 & FVC (Vowel)           & 0.850 ± 0.592	&0.895 ± 0.559	&0.833 ± 0.588	&0.883 ± 0.560	&0.885 ± 0.553	&\cellcolor{mypink}0.761 ± 0.544	&0.878 ± 0.550  &\textcolor{red}{\checkmark*}  \\
T17 & FEV1 (Vowel)           &\cellcolor{mypink}0.730 ± 0.497	&0.842 ± 0.559	&0.876 ± 0.561	&0.859 ± 0.541	&0.780 ± 0.542	&0.830 ± 0.561	&0.774 ± 0.554    &\textcolor{red}{~~~*}  \\
T18 & FEV1/FVC (Vowel)        &0.138 ± 0.166	&\cellcolor{mypink}0.130 ± 0.145	&0.131 ± 0.141	&0.137 ± 0.147	&0.132 ± 0.140	&0.136 ± 0.150	&\cellcolor{mypink}0.130 ± 0.138 &\textcolor{red}{\checkmark*}  \\
T19 & Breathing Rate        &2.714 ± 0.902	&2.605 ± 0.759	&2.641 ± 0.813	&2.650 ± 0.947	&2.636 ± 0.858	&2.525 ± 0.782	&\cellcolor{mypink}2.416 ± 0.885 &\textcolor{red}{\checkmark*} \\

  \bottomrule     
\end{tabular}
\end{adjustbox}
\label{tab:res:lung}
\vspace{-15pt}
\end{table}

% T13          & \cellcolor{mypink}{0.965 ± 0.589} & 1.545 ± 2.084 & 1.345 ± 0.792 & 1.138 ± 0.962 & 1.606 ± 1.312   & 1.023 ± 0.854   & 1.191 ± 0.721 \\
% T14          & 0.859 ± 0.815 & 1.738 ± 2.967 & 1.081 ± 0.720 & 1.130 ± 0.845 & 1.459 ± 1.074   & \cellcolor{mypink}{0.771 ± 0.752}   & 0.996 ± 0.732 \\
% T15          & 0.194 ± 0.397 & 0.279 ± 0.629 & \cellcolor{mypink}{0.143 ± 0.153} & 0.178 ± 0.151 & 0.155 ± 0.155   & 0.148 ± 0.165   & 0.155 ± 0.172 \\
% T16          & 0.724 ± 0.532 & 0.900 ± 1.377 & 0.983 ± 0.721 & 0.710 ± 0.585 & 1.737 ± 1.041   & 0.672 ± 0.535   & \cellcolor{mypink}{0.593 ± 0.414}  \\
% T17          & 0.605 ± 0.541 & 1.103 ± 1.466 & 0.960 ± 0.741 & 0.838 ± 0.694 & 1.488 ± 1.005   & 0.736 ± 0.566   & \cellcolor{mypink}{0.561 ± 0.348}  \\
% T18          & 0.179 ± 0.204 & 0.227 ± 0.301 & \cellcolor{mypink}{0.150 ± 0.184} & 0.276 ± 0.300 & 0.179 ± 0.127   & 0.220 ± 0.217   & 0.245 ± 0.185 \\
% T19          & 3.852 ± 1.060 & 2.611 ± 0.786 & 2.630 ± 0.832 & 2.615 ± 0.804 & 2.567 ± 0.785   & 2.623 ± 0.831   & \cellcolor{mypink}{2.537 ± 0.782} \\


 
% \begin{table}[t]
% \caption{MAE on lung function estimation tasks. A \textcolor{red}{lower MAE} score indicates better performance. The best performing model for each task is highlighted in pink.}
% \centering
% \begin{adjustbox}{width=0.95\textwidth,center} % {width=\columnwidth,center}
% \begin{tabular}{l|cccccccccc}
% \toprule
% Task $ \ \ \ \ \ $  & Opensmile     & VGGish        & AudioMAE      & CLAP          & \textbf{OPERA-CT} & \textbf{OPERA-CE} & \textbf{OPERA-GT}  & $\Delta$\\
%   \midrule
% T13          & \cellcolor{mypink}{0.965 ± 0.589} & 1.545 ± 2.084 & 1.345 ± 0.792 & 1.138 ± 0.962 & 1.606 ± 1.312   & 1.023 ± 0.854   & 1.191 ± 0.721 & -6.0 -1.7\% \\
% T14          & 0.859 ± 0.815 & 1.738 ± 2.967 & 1.081 ± 0.720 & 1.130 ± 0.845 & 1.459 ± 1.074   & \cellcolor{mypink}{0.771 ± 0.752}   & 0.996 ± 0.732 &  10.2 3.3\%\\
% T15          & 0.194 ± 0.397 & 0.279 ± 0.629 & \cellcolor{mypink}{0.143 ± 0.153} & 0.178 ± 0.151 & 0.155 ± 0.155   & 0.148 ± 0.165   & 0.155 ± 0.172 &  -3.5 -0.6\%\\
% T16          & 0.724 ± 0.532 & 0.900 ± 1.377 & 0.983 ± 0.721 & 0.710 ± 0.585 & 1.737 ± 1.041   & 0.672 ± 0.535   & \cellcolor{mypink}{0.593 ± 0.414} & 16.5 3.4\% \\
% T17          & 0.605 ± 0.541 & 1.103 ± 1.466 & 0.960 ± 0.741 & 0.838 ± 0.694 & 1.488 ± 1.005   & 0.736 ± 0.566   & \cellcolor{mypink}{0.561 ± 0.348} & 7.3 1.7\% \\
% T18          & 0.179 ± 0.204 & 0.227 ± 0.301 & \cellcolor{mypink}{0.150 ± 0.184} & 0.276 ± 0.300 & 0.179 ± 0.127   & 0.220 ± 0.217   & 0.245 ± 0.185 & -19.3\% -3.6\\
% T19          & 3.852 ± 1.060 & 2.611 ± 0.786 & 2.630 ± 0.832 & 2.615 ± 0.804 & 2.567 ± 0.785   & 2.623 ± 0.831   & \cellcolor{mypink}{2.537 ± 0.782} &  2.8 0.5\%\\

 
%   \bottomrule     
% \end{tabular}
% \end{adjustbox}
% \label{tab:res:lung}
% \end{table}

==> tables/event-level.tex <==
% \usepackage{color}
% \usepackage{tabularray}
\begin{table}[t]
\caption{Performance on respiratory event classification tasks. (Modalities: S: Snoring, L: Lung Sounds, M: Multiple).}
\centering
\begin{adjustbox}{width=520pt,center} % {width=\columnwidth,center}
\begin{tabular}{lccc|ccccccccc}
\toprule
\textbf{Dataset}         & \textbf{Task}                           & \textbf{Mod.} & \textbf{\#} & \textbf{Opensmile} & \textbf{VGGish} & \textbf{AudioMAE} & \textbf{CLAP} & \textbf{COLA-H} & \textbf{COLA-E} & \textbf{MAE-T} \\

  \midrule

ICBHI            & wheeze \& crackle detection                      & L   & 6898        & 0.615 ± 0.005      & 0.617 ± 0.002   & 0.597 ± 0.001     & \textbf{0.694 ± 0.001} & 0.571 ± 0.004          & 0.556 ± 0.001          & 0.574 ± 0.001  \\
HF Lung       & CAS \& DAS detection                            & L   & 6268        & 0.625 ± 0.010      & 0.550 ± 0.004   & 0.536 ± 0.002     & \textbf{0.717 ± 0.002 }         & 0.512 ± 0.002          & 0.553 ± 0.003          &   \\
ESC-50           & Event classification                    &    M   & 160         & 0.559 ± 0.062      & 0.749 ± 0.035   & 0.719 ± 0.011     & \textbf{1.000 ± 0.000} & 0.834 ± 0.016          & 0.904 ± 0.005          & 0.921 ± 0.009  \\
SSBPR      & Body position recognition &  S       &   7468          & 0.772 ± 0.005      & 0.657 ± 0.002   & 0.649 ± 0.001     & 0.702 ± 0.001          & \textbf{0.781 ± 0.000} & 0.769 ± 0.000          & 0.520 ± 0.012  \\


 
  \bottomrule     
\end{tabular}
\end{adjustbox}
\end{table}

==> tables/lungfunction.tex <==


\begin{table}[t]
\caption{Performance on lung function estimation tasks.}
\centering
\begin{adjustbox}{width=520pt,center} % {width=\columnwidth,center}
\begin{tabular}{llll|ccccccccc}
\toprule
 \textbf{Dataset}  $ \ \ \ \ \ \ \ \ \ \ \ \ \ \ $       & \textbf{Task}              $ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ $         & \textbf{Mod.} & \textbf{\#} & \textbf{Opensmile} & \textbf{VGGish} & \textbf{AudioMAE} & \textbf{CLAP} & \textbf{COLA-H} & \textbf{COLA-E} & \textbf{MAE-T} \\

  \midrule


MMlung           & FVC      & B   & 40          & \textbf{0.965 ± 0.589 }     & 1.545 ± 2.084   & 1.345 ± 0.792     & 1.138 ± 0.962 & 1.606 ± 1.312          & 1.023 ± 0.854          & 1.191 ± 0.721  \\
                 & FEV1   & B   & 40          & 0.859 ± 0.815      & 1.738 ± 2.967   & 1.081 ± 0.720     & 1.130 ± 0.845 & 1.459 ± 1.074          & \textbf{0.771 ± 0.752 }         & 0.996 ± 0.732  \\
                 & FEV1/FVC  & B   & 40          & 0.194 ± 0.397      & 0.279 ± 0.629   & \textbf{0.143 ± 0.153 }    & 0.178 ± 0.151 & 0.155 ± 0.155          & 0.148 ± 0.165          & 0.155 ± 0.172  \\
                 & FVC      & O      & 40          & 0.724 ± 0.532      & 0.900 ± 1.377   & 0.983 ± 0.721     & 0.710 ± 0.585 & 1.737 ± 1.041          & 0.672 ± 0.535          & \textbf{0.593 ± 0.414 } \\
                 & FEV1     & O      & 40          & 0.605 ± 0.541      & 1.103 ± 1.466   & 0.960 ± 0.741     & 0.838 ± 0.694 & 1.488 ± 1.005          & 0.736 ± 0.566          & \textbf{0.561 ± 0.348}  \\
                 & FEV1/FVC  & O      & 40          & 0.179 ± 0.204      & 0.227 ± 0.301   & \textbf{0.150 ± 0.184}     & 0.276 ± 0.300 & 0.179 ± 0.127          & 0.220 ± 0.217          & 0.245 ± 0.185  \\
NoseMic            & Respiratory rate (bpm)      & B             & 16/1297     & 3.012 ± 0.818           & 3.168 ± 1.038   & 3.242 ± 1.203           & 2.978 ± 0.729 & 2.999 ± 0.958   & 3.001 ± 0.829           & \textbf{2.943 ± 0.801}  \\

 
  \bottomrule     
\end{tabular}
\end{adjustbox}
\label{tab:res:lung}
\end{table}

==> tables/participant.tex <==
% \usepackage{color}
% \usepackage{tabularray}
\begin{table}[t]
\caption{Performance on health condition inference tasks. (Modalities: E: Exhalation, B: Breath, C: Cough, L: Lung Sounds)}
\centering
\begin{adjustbox}{width=520pt,center} % {width=\columnwidth,center}
\begin{tabular}{llll|ccccccccc}
\toprule
\textbf{Dataset}         & \textbf{Task}                           & \textbf{Mod.} & \textbf{\#} & \textbf{Opensmile} & \textbf{VGGish} & \textbf{AudioMAE} & \textbf{CLAP} & \textbf{COLA-H} & \textbf{COLA-E} & \textbf{MAE-T} \\

  \midrule
%  UK COVID-19       & Covid/Non-covid                        & E        & 2500                & 0.550                     & 0.580                  & 0.549                    & 0.565                    & 0.586                              & 0.551                       & \textbf{0.605}     \\
%  UK COVID-19       & Covid/Non-covid                          & C             & 2500                & 0.649                    & 0.557                 & 0.616                    & 0.648                    & \textbf{0.701}                     & 0.629                       & 0.677              \\
% COVID-19 Sounds          & Symptomatic/Healthy                     & B      & 4138                & 0.571                    & 0.571                 & 0.583                    & \textbf{0.611}           & 0.603                              & 0.610                        & 0.613              \\
% COVID-19 Sounds          & Symptomatic/Healthy                    & C      & 4138                & 0.633                    & 0.605                 & 0.659                    & 0.669                    & \textbf{0.680}                      & 0.665                       & 0.673              \\
% Coswara                  & Smoker/Non-smoker                       & C      & 948                 & 0.534                    & 0.507                 & 0.549                    & 0.680                     & \textbf{0.685}                     & 0.674                       & 0.650               \\
% Coswara                  & Female/Male                                  & C     & 2496                & 0.753                    & 0.606                 & 0.724                    & 0.742                    & \textbf{0.874}                     & 0.801                       & 0.825              \\
% CoughVID                 & Covid/Non-covid                         & C     & 6175                & 0.546                    & 0.602                 & 0.549                    & 0.603                    & \textbf{0.609}                     & 0.584                       & 0.575              \\
% CoughVID        & Female/Male                                 & C    & 7263                & 0.639                    & 0.608                 & 0.666                    & 0.684                    & \textbf{0.801}                     & 0.722                       & 0.762              \\
% KAUH   & Healthy/Obstructive             & L      & 234                 & 0.502                    & 0.505                 & 0.614                    & 0.703                    & 0.719                              & \textbf{0.742}              & 0.700                \\
% TR & COPD severity               &   L    & 504                 & 0.494                    & 0.590                  & 0.510                     & 0.635                    & 0.625                              & \textbf{0.683}              & 0.615              \\

UK COVID-19      & Covid/Non-covid     & E             & 2500        & 0.550_{\pm.015}      & 0.580 ± 0.001   & 0.549 ± 0.001     & 0.565 ± 0.001          & 0.586 ± 0.008 & 0.551 ± 0.010          & \textbf{0.605 ± 0.001}  \\
     & Covid/Non-covid     & C             & 2500        & 0.649 ± 0.006      & 0.557 ± 0.005   & 0.616 ± 0.001     & 0.648 ± 0.003          & \textbf{0.701 ± 0.002} & 0.629 ± 0.006          & 0.677 ± 0.001  \\
COVID-19 Sounds  & Symptomatic/Healthy & B             & 4138        & 0.571 ± 0.006      & 0.571 ± 0.003   & 0.583 ± 0.003     & 0.611 ± 0.006 & 0.603 ± 0.005          & 0.610 ± 0.004          & \textbf{0.613 ± 0.002}  \\
  & Symptomatic/Healthy & C             & 4138        & 0.633 ± 0.012      & 0.605 ± 0.004   & 0.659 ± 0.001     & 0.669 ± 0.002          & \textbf{0.680 ± 0.006} & 0.665 ± 0.001          & 0.673 ± 0.001  \\
  CoughVID         & Covid/Non-covid     & C             & 6175        & 0.546 ± 0.008      & 0.602 ± 0.001   & 0.549 ± 0.005     & 0.603 ± 0.013          & \textbf{0.609 ± 0.004} & 0.584 ± 0.003          & 0.575 ± 0.006  \\
        & Female/Male         & C             & 7263        & 0.639 ± 0.010      & 0.608 ± 0.000   & 0.666 ± 0.002     & 0.684 ± 0.002          & \textbf{0.801 ± 0.000} & 0.722 ± 0.004          & 0.762 ± 0.001  \\
ICBHI        & COPD/Healthy    & L   & 828  &       0.579 ± 0.043	 &  0.605 ± 0.077 &  	0.886 ± 0.017	 &  \textbf{0.933 ± 0.005} &  	0.855 ± 0.012 &  	0.872 ± 0.011 & 0.741 ± 0.011\\
 \midrule
Coswara          & Smoker/Non-smoker   & C             & 948         & 0.534 ± 0.06       & 0.507 ± 0.027   & 0.549 ± 0.022     & 0.680 ± 0.009          & \textbf{0.685 ± 0.012} & 0.674 ± 0.013          & 0.650 ± 0.005  \\
        & Female/Male         & C             & 2496        & 0.753 ± 0.008      & 0.606 ± 0.003   & 0.724 ± 0.001     & 0.742 ± 0.001          & \textbf{0.874 ± 0.000} & 0.801 ± 0.002          & 0.825 ± 0.001  \\


KAUH             & Healthy/Obstructive & L             & 234         & 0.502 ± 0.08       & 0.505 ± 0.11    & 0.614 ± 0.040     & 0.703 ± 0.036          & 0.719 ± 0.018          & \textbf{0.742 ± 0.014} & 0.700 ± 0.013  \\
TR               & COPD severity       & L             & 504         & 0.494 ± 0.054      & 0.590 ± 0.034   & 0.510 ± 0.021     & 0.635 ± 0.040          & 0.625 ± 0.038          & \textbf{0.683 ± 0.007} & 0.615 ± 0.019  \\

SSBPR      & Body position recognition &  S       &   7468          & 0.772 ± 0.005      & 0.657 ± 0.002   & 0.649 ± 0.001     & 0.702 ± 0.001          & \textbf{0.781 ± 0.000} & 0.769 ± 0.000          & 0.520 ± 0.012  \\
  \bottomrule     
\end{tabular}
% Performance on health status inference tasks.
\end{adjustbox}
\label{tab:res:health}
\end{table}

==> tables/regression.tex <==
\begin{table}[t]
\caption{MAE for Task 19.}
\centering
\begin{adjustbox}{width=0.6\textwidth,center} % {width=\columnwidth,center}
\begin{tabular}{l|cccccccccc}
\toprule
Model             & \textbf{OPERA-CT} & \textbf{OPERA-CE} & \textbf{OPERA-GT} \\
  \midrule
Linear regression  & 2.567 ± 0.785   & 2.622 ± 0.803   & 2.537 ± 0.782 \\
Transformer regression  & 2.501 ± 0.842 & 2.631 ± 0.828  & 2.318 ± 0.733 \\
  \bottomrule     
\end{tabular}
\end{adjustbox}
\label{tab:res:lung_2}
\end{table}
